Implicit Class-Conditioned Domain Alignment for Unsupervised Domain Adaptation

We present an approach for unsupervised domain adaptation---with a strong focus on practical considerations of within-domain class imbalance and between-domain class distribution shift---from a class-conditioned domain alignment perspective. Current methods for class-conditioned domain alignment aim to explicitly minimize a loss function based on pseudo-label estimations of the target domain. However, these methods suffer from pseudo-label bias in the form of error accumulation. We propose a method that removes the need for explicit optimization of model parameters from pseudo-labels directly. Instead, we present a sampling-based implicit alignment approach, where the sample selection procedure is implicitly guided by the pseudo-labels. Theoretical analysis reveals the existence of a domain-discriminator shortcut in misaligned classes, which is addressed by the proposed implicit alignment approach to facilitate domain-adversarial learning. Empirical results and ablation studies confirm the effectiveness of the proposed approach, especially in the presence of within-domain class imbalance and between-domain class distribution shift.

==> ablation_and_visda.tex <==
\begin{figure*}[ht]
\begin{minipage}[!t]{0.32\linewidth}
    \centering
    \includegraphics[width=0.94\textwidth]{figures/diversity_ablation.pdf}
    \captionsetup{font=footnotesize}
    \captionof{figure}{Impact of diversity and~alignment}
    \label{fig:impact_of_cls_diversity}
\end{minipage}\hfill
\begin{minipage}[!t]{0.32\linewidth}
\vspace{0pt}
    %\centering
    \includegraphics[width=0.94\textwidth]{figures/calibration_robustness_boxplot.pdf}
    \captionof{figure}{
    Impact of pseudo-label errors
    %Implicit alignment is more robust to pseudo-label errors  than explicit alignment for Ar$\rightarrow$Pr,~Office-Home~(standard).
    }
    \label{fig:robustness_to_calibration}
\end{minipage}\hfill
\begin{minipage}[!t]{0.35\linewidth}
\vspace{0pt}\raggedright
\addtolength{\tabcolsep}{-4pt} 
%\centering
\renewcommand{\arraystretch}{1.45}
\scalebox{0.9}{
\begin{tabular}{cc}
\toprule
method & acc.~(\%) \\\midrule
JAN~\cite{long2017deep} & 61.6 \\
GTA\cite{sankaranarayanan2018generate} & 69.5 \\
MCD~\cite{saito2018maximum} & 69.8 \\
CDAN~\cite{long2018conditional} & 70.0 \\
MDD~\cite{pmlr-v97-zhang19i} & 74.6 \\
%MDD~(re-implementation) & 68.7 \\
MDD+Explicit Alignment & 67.1 \\
\textbf{MDD+Implicit Alignment} & \textbf{75.8} \\\bottomrule
\end{tabular}
}
\captionof{table}{VisDA2017 target accuracy (ResNet-50)}
\label{tab:visda}
\end{minipage}\hfill
\end{figure*}

==> tables/mdd_ablation_table.tex <==
\begin{table}[]
    \centering
    \addtolength{\tabcolsep}{+4pt} 
\scalebox{0.9}{
\begin{tabular}[!t]{cccc}
\toprule
 & \multicolumn{2}{c}{Alignment options} & \\ \cmidrule{2-3}
Domains                                 & masking               & sampling              & Accuracy~(\%) \\\midrule
\multirow{4}{*}{Rw$\shortrightarrow$Cl} & $\times$   & $\times$    & 44.8                 \\
                                        & $\surd$   & $\times$    & 44.8                 \\
                                        & $\times$   & $\surd$    & 47.4                 \\
                                        & $\surd$   & $\surd$    & \textbf{50.0}                 \\\midrule
\multirow{4}{*}{Pr$\shortrightarrow$Rw} & $\times$   & $\times$    & 69.3                 \\
                                        & $\surd$   & $\times$    & 72.7                 \\
                                        & $\times$   & $\surd$    & 72.0                 \\
                                        & $\surd$   & $\surd$    & \textbf{74.2}       \\\bottomrule         

\end{tabular}
}
\caption{The impact of different implicit alignment options, i.e., masking in the MDD estimation and sampling class-aligned minibatches, on Office-Home~(RS-UT). Evaluated on average accuracy per-class.}
\label{tab:alignment-ablation}
\end{table}
